Damage Location in Mechanical Structures by Multi-Objective Pattern Search

We propose a multi-objective global pattern search algorithm for the task of locating and quantifying damage in flexible mechanical structures. This is achieved by identifying eigenfrequencies and eigenmodes from measurements and matching them against the results of a finite element simulation model, which leads to a nonsmooth nonlinear bi-objective parameter estimation problem. A derivative-free optimization algorithm is required since the problem is nonsmooth and also because complex mechanical simulation models are often solved using commercial black-box software. Moreover, the entire set of non-dominated solutions is of interest to practitioners. Most solution approaches published to date are based on meta-heuristics such as genetic algorithms. The proposed multi-objective pattern-search algorithm provides a mathematically well-founded alternative. It features a novel sorting procedure that reduces the complexity in our context. Test runs on two experimental structures with multiple damage scenarios are used to validate the approach. The results demonstrate that the proposed algorithm yields accurate damage locations and requires moderate computational resources. From the engineer's perspective it represents a promising tool for structural health monitoring.

==> abbr.tex <==
% Abbreviations -- requires package xspace

\newcommand\abbrfont{}

\newcommand\abbr[1][abbrev]{{\abbrfont{#1.}}\xspace}
\newcommand\abbrev{\abbr}
\providecommand\ca{\abbr[ca]}% Also in abk.tex.
\newcommand\cf{\abbr[cf]}
\newcommand\eg{\abbr[e.g]}
\providecommand\etal{\abbr[et~al]}% Also in abk.tex.
\providecommand\etc{\abbr[etc]}% Also in abk.tex.
\newcommand\ie{\abbr[i.e]}
\newcommand\resp{\abbr[resp]}
\providecommand\vs{\abbr[vs]}% Also in abk.tex.
\newcommand\Wlog{\abbr[w.l.o.g]}% \wlog is an internal logging command.
\newcommand\wrt{\abbr[w.r.t]}


==> abk.tex <==
% Abkürzungen -- benötigt package xspace

\newcommand\abkfont{}

\newcommand\Abk[1][Abk]{{\abkfont{#1.}}\xspace}
\newcommand\bzw{\Abk[bzw]}
\newcommand\bzgl{\Abk[bzgl]}
\providecommand\ca{\Abk[ca]}% Also in abbr.tex.
\let\TeXdh\dh
\renewcommand\dh{\Abk[d.\,h]}% Now \dh, not \ie: original \dh mostly unused.
\PackageInfo{abk}{Redefining \string\dh\space
 (use \string\TeXdh\space for TeX \string\dh)}
\providecommand\Dr{\Abk[Dr]}
\providecommand\DrIng{\Abk[Dr.-Ing]}
\newcommand\engl{\Abk[engl]}
\providecommand\etal{\Abk[et~al]}% Also in abbr.tex.
\providecommand\etc{\Abk[etc]}% Also in abbr.tex.
\newcommand\evtl{\Abk[evtl]}
\newcommand\ggf{\Abk[ggf]}
\newcommand\iA{\Abk[i.\,A]}
\newcommand\MEd{\Abk[M.\,Ed]}
\newcommand\MSc{\Abk[M.\,Sc]}
\newcommand\OBdA{\Abk[O.\,B.\,d.\,A]}
\newcommand\oBdA{\Abk[o.\,B.\,d.\,A]}
\newcommand\oE{\Abk[o.\,E]}
\newcommand\og{\Abk[o.\,g]}
\providecommand\Prof{\Abk[Prof]}
\newcommand\sog{\Abk[sog]}
\newcommand\ua{\Abk[u.\,a]}
\newcommand\usw{\Abk[usw]}
\newcommand\vgl{\Abk[vgl]}
\newcommand\wiss{\Abk[wiss]}
\providecommand\vs{\Abk[vs]}% Also in abbr.tex.
\newcommand\zB{\Abk[z.\,B]}
\newcommand\zT{\Abk[z.\,T]}


==> code-names.tex <==
% Code names -- requires packages xspace and relsize

\providecommand\sfnamesize{\relsize{0}}
\providecommand\sfname[1]{\textsf{\sfnamesize#1}\xspace}

\newcommand\plusplus{\raisebox{0.15ex}{++}}
\newcommand\ALADIN{\sfname{ALADIN}}
\newcommand\AMPL{\sfname{AMPL}}
\newcommand\BARON{\sfname{BARON}}
\newcommand\Bash{\sfname{Bash}}
\newcommand\BGL{\sfname{BGL}}
\newcommand\BLAS{\sfname{BLAS}}
\newcommand\Bonmin{\sfname{Bonmin}}
\newcommand\boost{\sfname{boost}}
\newcommand\Boost{\sfname{Boost}}
\newcommand\BoostMPI{\sfname{Boost.MPI}}
\newcommand\langC{\sfname{C}}
\newcommand\CC{\sfname{C\plusplus}}
\newcommand\Cpp{\CC}
\newcommand\CCEleven{\sfname{C\plusplus 11}}
\newcommand\CppEleven{\CCEleven}
\newcommand\CCFourteen{\sfname{C\plusplus 14}}
\newcommand\CppFourteen{\CCFourteen}
\newcommand\Clean{\sfname{Clean}}
\newcommand\clean{\sfname{clean}}
\newcommand\CleanIPM{\sfname{Clean::IPM}}
\newcommand\cleanIPM{\sfname{clean::ipm}}
\newcommand\CONOPT{\sfname{CONOPT}}
\newcommand\CONOPTfour{\sfname{CONOPT4}}
\newcommand\CPLEX{\sfname{CPLEX}}
\newcommand\CUTE{\sfname{CUTE}}
\newcommand\CUTEr{\sfname{CUTEr}}
\newcommand\CUTEst{\sfname{CUTEst}}
\newcommand\dealII{\sfname{deal.II}}
\newcommand\DeSiO{\sfname{DeSiO}}
\newcommand\DICOPT{\sfname{DICOPT}}
\newcommand\DOpElib{\sfname{DOpElib}}
\newcommand\DOM{\sfname{DOM}}
\newcommand\Doxygen{\sfname{Doxygen}}
\newcommand\EPANET{\sfname{EPANET}}
\newcommand\Excel{\sfname{Excel}}
\newcommand\FilterSQP{\sfname{FilterSQP}}
\newcommand\filtermpec{\sfname{filtermpec}}
\newcommand\GAMS{\sfname{GAMS}}
\newcommand\GasLib{\sfname{GasLib}}
\newcommand\GCC{\sfname{GCC}}
\newcommand\Gurobi{\sfname{Gurobi}}
\newcommand\Fortran{\sfname{Fortran}}
\newcommand\FortranSS{\sfname{Fortran 77}}
\newcommand\iGNO{\sfname{iGNO}}
\newcommand\Ipopt{\sfname{Ipopt}}
\newcommand\IPM{\sfname{IPM}}
\newcommand\Java{\sfname{Java}}
\newcommand\KNITRO{\sfname{KNITRO}}
\newcommand\KNITRODIRECT{\sfname{KNITRO/DIRECT}}
\newcommand\KNITROCG{\sfname{KNITRO/CG}}
\newcommand\LaGO{\sfname{LaGO}}
\newcommand\Lamatto{\sfname{LaMaTTO\plusplus}}
\newcommand\LAPACK{\sfname{LAPACK}}
\newcommand\Liwacom{\sfname{Liwacom}}
\newcommand\LOQO{\sfname{LOQO}}
\newcommand\MacMPEC{\sfname{MacMPEC}}
\newcommand\Matlab{\sfname{Matlab}}
\newcommand\MINLPLib{\sfname{MINLPLib}}
\newcommand\MINOS{\sfname{MINOS}}
\newcommand\MOSEK{\sfname{MOSEK}}
\newcommand\MPC{\sfname{MPC}}
\newcommand\MPI{\sfname{MPI}}
\newcommand\MSIPM{\sfname{MSIPM}}
\newcommand\MSKKT{\sfname{MSKKT}}
\newcommand\MSSQP{\sfname{MSSQP}}
\newcommand\MSTOP{\sfname{MSTOP}}
\newcommand\OOPS{\sfname{OOPS}}
\newcommand\openMPI{\sfname{Open MPI}}
\newcommand\Pardiso{\sfname{Pardiso}}
\newcommand\Python{\sfname{Python}}
\newcommand\SCIP{\sfname{SCIP}}
\newcommand\Simone{\sfname{SIMONE}}
\newcommand\SNOPT{\sfname{SNOPT}}
\newcommand\SQP{\sfname{SQP}}
\newcommand\TreeKKT{\sfname{TreeKKT}}
\newcommand\Xerces{\sfname{Xerces}}
\newcommand\XML{\sfname{XML}}
\newcommand\Zimpl{\sfname{Zimpl}}


==> math-fields.tex <==
% Math fields -- requires amsfonts

\newcommand{\field}{\mathbb}

% "natural" names
\newcommand{\complex}{\field{C}}
\newcommand{\quaternions}{\field{H}}
\newcommand{\naturals}{\field{N}}
\newcommand{\polynomials}{\field{P}}
\newcommand{\rationals}{\field{Q}}
\newcommand{\reals}{\field{R}}
\newcommand{\integers}{\field{Z}}

% alternative names
\newcommand{\numsetC}{\complex}
\newcommand{\numsetH}{\quaternions}
\newcommand{\numsetN}{\naturals}
\newcommand{\numsetQ}{\rationals}
\newcommand{\numsetR}{\reals}
\newcommand{\numsetZ}{\integers}

% short names
\makeatletter
\@ifundefined{C}{\newcommand{\C}{\complex}}
{\PackageInfo{math-fields}{Use \string\field{C} for complex numbers;
 \MessageBreak command \string\C\space already defined}{}}
\makeatother
\newcommand{\N}{\naturals}
\newcommand{\Q}{\rationals}
\newcommand{\R}{\reals}
\newcommand{\Z}{\integers}
\newcommand{\Poly}{\polynomials}% deprecated: NuMa scripts


==> math-std.tex <==
% Standard math definitions -- requires amsmath

\newcommand\const{\textup{const}}
\newcommand\qtext{\quad\text}
\newcommand\textq[1]{\text{#1}\quad}
\newcommand\qtextq{\quad\textq}
\newcommand\st{\textup{s.t.}}
\newcommand\stq{\st\quad}
\newcommand\qst{\quad\st}
\newcommand\qstq{\qst\quad}

\makeatletter
\newcommand\fcdot{\,\cdot\,}
\newcommand\ifgiven[3]{\def\fc@rg{#1}\ifx\fc@rg\empty#3\else#2\fi}
\newcommand\fcarg[1]{\ifgiven{#1}\fc@rg\fcdot}
\makeatother
\newcommand\abs[1]{\lvert\fcarg{#1}\rvert}
\newcommand\Abs[1]{\left\lvert#1\right\rvert}
\newcommand\tfracabs[2]{\abs{#1}/\abs{#2}}
\newcommand\fracabs[2]{\frac{\abs{#1}}{\abs{#2}}}
\newcommand\fracAbs[2]{\frac{\Abs{#1}}{\Abs{#2}}}
\newcommand\tabsfrac\tfracabs
\newcommand\absfrac\fracabs
\newcommand\Absfrac\fracAbs
\newcommand\card\abs
\newcommand\Card\Abs
\newcommand\ceil[1]{\lceil\fcarg{#1}\rceil}
\newcommand\Ceil[1]{\left\lceil#1\right\rceil}
\newcommand\pcolon{\mathpunct:}
\newcommand\defsep\pcolon% alternative: \mid
\newcommand\defset[3][\defsep]{\set{#2#1#3}}
\newcommand\Defset[3][\defsep]{\Set{#2#1#3}}
\newcommand\EEmult\cdot% alternative: \times
\newcommand\EE[1][\EEmult]{#1 10^}
\newcommand\floor[1]{\lfloor\fcarg{#1}\rfloor}
\newcommand\Floor[1]{\left\lfloor#1\right\rfloor}
\newcommand\Inv[1]{#1^{-1}}
\newcommand\HInv[1]{#1\ihr}% hermitian inverse
\newcommand\TInv[1]{#1\itp}% transpose inverse
\newcommand\norm[2][]{\lVert\fcarg{#2}\rVert\optsb{#1}}
\newcommand\Norm[2][]{\left\lVert#2\right\rVert\optsb{#1}}
\newcommand\tfracnorm[3][]{\norm[#1]{#2}/\norm[#1]{#3}}
\newcommand\fracnorm[3][]{\frac{\norm[#1]{#2}}{\norm[#1]{#3}}}
\newcommand\fracNorm[3][]{\frac{\Norm[#1]{#2}}{\Norm[#1]{#3}}}
\newcommand\tnormfrac\tfracnorm
\newcommand\normfrac\fracnorm
\newcommand\Normfrac\fracNorm
\newcommand\tfracnormpow[4][]{\norm[#1]{#2}^{#4}/\norm[#1]{#3}^{#4}}
\newcommand\fracnormpow[4][]{\frac{\norm[#1]{#2}^{#4}}{\norm[#1]{#3}^{#4}}}
\newcommand\fracNormpow[4][]{\frac{\Norm[#1]{#2}^{#4}}{\Norm[#1]{#3}^{#4}}}
\newcommand\pfrac[2]{\frac{\partial#1}{\partial#2}}
\newcommand\ppfrac[3]{\pfrac{^2#1}{#2\partial#3}}
\newcommand\set[1]{\{#1\}}
\newcommand\Set[1]{\left\{#1\right\}}
\newcommand\snorm[2][]{\lvert\!\lvert\!\lvert
  \fcarg{#2}\rvert\!\rvert\!\rvert\optsb{#1}}
\newcommand\Snorm[2][]{\left\lvert\!\left\lvert\!\left\lvert
  #2\right\rvert\!\right\rvert\!\right\rvert\optsb{#1}}
\newcommand\sprod[3][]{\langle\fcarg{#2},\fcarg{#3}\rangle\optsb{#1}}
\newcommand\Sprod[3][]{\left\langle#2,#3\right\rangle\optsb{#1}}

\newcommand\hrchar{H}
\newcommand\tpchar{T}
\newcommand\hr{^\hrchar}% hermitian transpose
\newcommand\tp{^\tpchar}
\newcommand\ihr{^{-\hrchar}}
\newcommand\itp{^{-\tpchar}}
\newcommand\tadj[1]{\mskip#1\thinmuskip}% adjust space
\newcommand\hra[1][0]{^{\tadj{#1}\hrchar}}
\providecommand\tpa[1][0]{^{\tadj{#1}\tpchar}}% Conflict with siamart190516.cls.
\newcommand\ihra[1][0]{^{\tadj{#1}{-}\hrchar}}
\newcommand\itpa[1][0]{^{\tadj{#1}{-}\tpchar}}
\newcommand\tpfrac[2]{\tfrac{\partial#1}{\partial#2}}
\newcommand\tppfrac[3]{\tpfrac{^2#1}{#2\partial#3}}
\newcommand\without{\setminus\set}
\newcommand\Without{\setminus\Set}

\newcommand\lbound{-}
\newcommand\ubound{+}
\newcommand\splb{^{\lbound}}
\newcommand\spub{^{\ubound}}
\newcommand\sblb{_{\lbound}}
\newcommand\sbub{_{\ubound}}
\newcommand\bounds[1]{\ensuremath{[#1\splb,#1\spub]}}
\newcommand\Bounds[1]{\ensuremath{\left[#1\splb,#1\spub\right]}}

\newcommand\Strut{\rule[2.5555ex]{0pt}{0pt}}% ~1.1em
\newcommand\Hline{\hline\Strut}

\newcommand\optsb[1]{\ifgiven{#1}{_{#1}}{}}
\newcommand\optsp[1]{\ifgiven{#1}{^{#1}}{}}
\newcommand\optindex[1]{\ifgiven{#1}{,#1}{}}
\newcommand\optmathsb\optsb
\newcommand\optmathsp\optsp
\newcommand\opttextsb[1]{\optsb{\textup{#1}}}
\newcommand\opttextsp[1]{\optsp{\textup{#1}}}
\newcommand\optmathindex\optindex
\newcommand\opttextindex[1]{\optindex{\textup{#1}}}

\newcommand\define{\mathrel{{\mathop:}{=}}}
\newcommand\enifed{\mathrel{{=}{\mathop:}}}


==> math-symbols.tex <==
% Math symbols -- requires amsmath

% Redefine some macros in math mode. Keep text mode definitions.
\let\TeXbar\_   % underscore -> \bar
\let\TeXhat\^   % undefined  -> \hat
\let\TeXtilde\~ % undefined  -> \tilde
\let\TeXcolon\: % \tmspace+\medmuskip{.2222em} -> \colon
\makeatletter
\newcommand\mcs@cc[3]{\leavevmode\ifmmode#1{#3}\else#2{#3}\fi}
\renewcommand\_{\mcs@cc\bar\TeXbar}
\renewcommand\^{\mcs@cc\hat\TeXhat}
\renewcommand\~{\mcs@cc\tilde\TeXtilde}
\renewcommand\:{\mcs@cc\colon\TeXcolon\relax}
\makeatother
\PackageInfo{math-symbols}{Redefining
 \string\_, \string\^, \string\~, \string\: in math mode.
 \MessageBreak Keeping text mode definitions.
 \MessageBreak Saving original commands as \string\TeXbar, \string\TeXhat,
 \MessageBreak \string\TeXtilde, \string\TeXcolon}

\newcommand\0\emptyset
\newcommand\bigM{M}
\newcommand\bigO{O}
\newcommand\smallo{o}
\newcommand\oo\infty
\newcommand\ox\otimes
\newcommand\x\times

\newcommand\itxt{\textup}% text in math indices
\newcommand\tsb[1]{_{\itxt{#1}}}% text subindex
\newcommand\tsp[1]{^{\itxt{#1}}}% text superindex

\newcommand\boundary\partial
\newcommand\cond\kappa
\newcommand\condabs{\cond\tsb{abs}}\newcommand\abscond\condabs
\newcommand\condrel{\cond\tsb{rel}}\newcommand\relcond\condrel
\newcommand\convrad\rho
\newcommand\eps\epsilon
\newcommand\veps\varepsilon
\newcommand\epsM{\veps\tsb{M}}
\let\epsmach\epsM
\newcommand\specrad\rho
\newcommand\spectrum\sigma
\newcommand\uvec{\mathbf1}

% Some arrows.
\newcommand\larrow\leftarrow
\newcommand\rarrow\to% \rightarrow
\newcommand\swap\leftrightarrow
\newcommand\lrarrow\swap
\newcommand\Larrow\longleftarrow
\newcommand\Rarrow\longrightarrow
\newcommand\LRarrow\longleftrightarrow
\newcommand\xlarrow\xleftarrow
\newcommand\xrarrow\xrightarrow
\newcommand\lArrow\Leftarrow
\newcommand\rArrow\Rightarrow

% Right-shifted relation symbols for alignment with :=
\newcommand\crel[1]{\mathrel{\hphantom:{#1}}}
\newcommand\isom{\crel\cong}
\newcommand\eqls{\crel=}


==> matrix.tex <==
% Matrices and column vectors -- requires amsmath

% Default space between array and delimiters.
\newcommand\matmargin{\,}
\newcommand\colmargin{\,}

% Separation lines.
\providecommand\vsl{|}
\providecommand\hsl{\hline}

% General delimited arrays: choose margin, format, delimiters.
% \Xmat{margin}{format}{ldelim}{rdelim}{entries}
\newcommand\Xmat[5][\matmargin]{%
  \left#3\begin{array}{@{#1}#2@{#1}}#5\end{array}\right#4}

% General matrices and vectors: choose margin, alignment, delimiters, ncol.
% ('<', '>' stand for ldelim, rdelim; last two args processed by \Xmat.)
% \xddmat[margin]{alignment}<nc1 nc2 nc3>{entries} (cols separated by |)
% \xdmat[margin]{alignment}<ncol1 ncol2>{entries} (cols separated by |)
% \xmat[margin]{alignment}<ncol>{entries}
% \xcol{margin}(alignment){entries}
\newcommand\xddmat[6][\matmargin]{
  \Xmat[#1]{*{#4}{#2}|*{#5}{#2}|*{#6}{#2}}{#3}}
% \Xmat[#1]{*{#4}{#2}\vsl*{#5}{#2}\vsl*{#6}{#2}}{#3}}
\newcommand\xdmat[5][\matmargin]{\Xmat[#1]{*{#4}{#2}|*{#5}{#2}}{#3}}
%\newcommand\xdmat[5][\matmargin]{\Xmat[#1]{*{#4}{#2}\vsl*{#5}{#2}}{#3}}
\newcommand\xmat[4][\matmargin]{\Xmat[#1]{*{#4}{#2}}{#3}}
\newcommand\xcol[3]{\Xmat[#1]{#3}{#2}}

% Standard matrices and vectors: choose alignment, delimiters, ncol.
\newcommand\lddmat{\xddmat[\matmargin]{l}}% \ldmat<nc1 nc2 nc3>{entries}
\newcommand\cddmat{\xddmat[\matmargin]{c}}% \cdmat<nc1 nc2 nc3>{entries}
\newcommand\rddmat{\xddmat[\matmargin]{r}}% \rdmat<nc1 nc2 nc3>{entries}
\newcommand\ddmat{\cddmat}
\newcommand\ldmat{\xdmat[\matmargin]{l}}% \ldmat<ncol1 ncol2>{entries}
\newcommand\cdmat{\xdmat[\matmargin]{c}}% \cdmat<ncol1 ncol2>{entries}
\newcommand\rdmat{\xdmat[\matmargin]{r}}% \rdmat<ncol1 ncol2>{entries}
\newcommand\dmat{\cdmat}
\newcommand\lmat{\xmat[\matmargin]{l}}% \lmat<ncol>{entries}
\newcommand\cmat{\xmat[\matmargin]{c}}% \cmat<ncol>{entries}
\newcommand\rmat{\xmat[\matmargin]{r}}% \rmat<ncol>{entries}
\newcommand\mat{\cmat}
\newcommand\col{\xcol{\colmargin}}% \col<alignment>{entries}

